A Learning Framework for Distribution-Based Game-Theoretic Solution Concepts

The past few years have seen several works on learning economic solutions from data; these include optimal auction design, function optimization, stable payoffs in cooperative games and more. In this work, we provide a unified learning-theoretic methodology for modeling such problems, and establish tools for determining whether a given economic solution concept can be learned from data. Our learning theoretic framework generalizes a notion of function space dimension -- the graph dimension -- adapting it to the solution concept learning domain. We identify sufficient conditions for the PAC learnability of solution concepts, and show that results in existing works can be immediately derived using our methodology. Finally, we apply our methods in other economic domains, yielding a novel notion of PAC competitive equilibrium and PAC Condorcet winners.

==> document.tex <==
%Single peaked preferences assume that there is some linear order $>$ over the candidates; for every voter $i$ there is some candidate $c_i$, where if $c'>c''>c_i$ or $c_i>c''>c'$ implies that $c''\succ c'$. Single-crossing preferences, on the other hand, assume that there is some ordering of the {\em voters} $>$ such that for every two candidates $c',c''$ there is some voter $i^*$ such that for every $i< i^*$, $c'\succ_i c''$ and for every $i^* \ge i$ $c'' \succ_i c'$ (for further reading see \citet{elkind2017structured}). 
%\begin{corollary}
%If the preference profile class $\HC$ is single-peaked or single-crossing, $\probleminstance_{\Cond}(\HC)$ is efficiently PAC solvable with sample complexity $\frac{1}{\epsilon}log\frac{1}{\delta}$.
%\end{corollary}
%\iffalse
%\begin{proof}
%	Theorem~\ref{thm:sample-condorcet} establishes that $\Sd(\probleminstance_{\Cond}(\HC))=1$. Given a sample $T$ of $m$ candidates, under single-peaked and single-crossing domains, we are guaranteed that there exists some candidate in $T$ that beats all of the candidates in $T$ in a pairwise election (simply observe the tournament graph induced by the candidates in $T$). This candidate can be found in $\cal O(m^2$ time over a sample of $m$ candidates, and we are done. 
%\end{proof}
%\fi
%\begin{definition}
%Given a preference profile of voters, define the tournament graph over set of candidates $C$, as $T = (C, E)$, where $E$ is the set of directed edges such that $u_ij \in E$ iff a majority of voters prefer $c_j$ over $c_i$. 
%\end{definition}
However, for many families of preferences, a Condorcet winner may not exist; we discuss this case in the appendix.
%An important limitation in voting theory is that Condorcet winners may not always exist, even when the number of candidates is small; this is due to the existence of Condorcet cycles (or Condorcet paradoxes). In fact, as discussed below, whenever the Condorcet winner is known to exist amongst a sample $C' \in C$, the problem is equivalent to the argmax problem discussed in Corollary \ref{corr:argmax}. However, as shown in Section \ref{sec:agnostic}, the graph dimension is still useful as a means to estimate, within $\pm \eps$ with high confidence, the behavior of a candidate in pairwise elections using a small empirical sample. 
%\begin{theorem}
%Let $k$ be the largest number of candidates, such that for some tournament graph in $\HC$, every pair among them is part of some $3$-cycle. Then $\Sd(\probleminstance_{\Cond}) \leq log_2 (k+2)$.
%\end{theorem}

\begin{tushantcomment}
Proof hidden.
\end{tushantcomment}

\iffalse
\begin{proof}
Let us assume that there is a set of size $d$, $C_0 \in C$, that is shattered. Then by definition of shattering, there exists $2^d$ different candidates corresponding to every subset of $C_0$, such that for $f \in 2^{C_0}$ there exists a candidate $c_f \in C$, such that $c_1 \in C_0$ beats $c_f$ in the tournament graph if and only if $f(c_1) = 1$.

Let us focus on $2^d - 2$ of these candidates, corresponding to all non-trivial functions $f \in 2^{C_0}$ (let us, for now, ignore the functions that assign a constant value (of $0$ or $1$) to all candidates in $C_0$). Then, for every pair of these functions $f_1$ and $f_2$, there exists a candidate $c_1 \in C_0$ such that $f_1(c_1) = 1$ and $f_2(c_1) = 0$, and a candidate $c_2$ such that $f_1(c_2) = 0$ and $f_2(c_2) = 1$. This implies the existence of a directed path of length at most $2$ from $c_{f_1}$ to $c_{f_2}$, and vice versa. Since, in a tournament graph, either the edge $c_{f_1}\to c_{f_2}$ or $c_{f_2}\to c_{f_1}$ exists, we know that $c_{f_1}$ and $c_{f_2}$ are members of some $3$-cycle. Since this is true for all such $c_f$'s, we know that $2^d - 2$ is less than or equal to largest number of candidates, such that for some tournament graph in $\HC$, every pair amongst them is part of some $3$-cycle. 
\end{proof}
\fi

==> vctheory.tex <==
\section{A Unified Framework for Learning Statistical Solution Concepts}\label{sec:framework}

\subsection{Introduction to the framework}\label{subsec:framework}

All of the problems we study share a common thread: we are given a problem domain (cooperative games, markets, elections), and are interested in identifying a {\em statistical solution} to the problem: a payoff division that is likely in the core, an outcome that is likely to be a market equilibrium, or a candidate that is likely to be a Condorcet winner. We now present a unified framework to discuss these domains.  
\begin{definition}\label{def:stat-solutionconcept}
An instance of the \probleminstancename problem (denoted $\probleminstance$) is given by a tuple $\probleminstance = (\cal X_{\probleminstance}, \cal Y_{\probleminstance}, \G_{\probleminstance}, \Sol_{\probleminstance}, \lambda_{\probleminstance})$; we omit the problem space $\probleminstance$ subscript when it is clear from context. Here:
\begin{itemize}
    \item $\cal X$ is the instance space.
    \item $\cal Y$ is the codomain (or label) space.
    \item $\G \subseteq \cal Y^{\cal X}$ is the function space: this is simply a subclass of the domain of interest.
    \item $\Sol$ is the solution space
    \item The function $\lambda : \cal X \times \G \times \Sol \rightarrow \lbrace 0,1 \rbrace$ measures local loss.
\end{itemize}

\end{definition}
In classic PAC learning, the solution space $\Sol = \G$, and $\lambda(x,g,s) = 0$ if and only if $g(x) = s(x)$. In the empirical maximum example, $\Sol = \R$, and $\lambda(x,g,s) = 0$ if and only if $s \ge g(x)$. 
In TU cooperative games, $\cal X_\TU$ is the set of all subsets of $N$; $\cal Y_\TU = \R$, $\G_\TU$ would be some subclass of cooperative games (e.g. weighted voting games, or network flow games); $\Sol_\TU\subseteq \R^n$ is the the set of vectors satisfying efficiency and individual rationality. Finally, given some set $S \in \cal X_\TU = 2^N$, a cooperative game $v \in \G_\TU$ and a payoff division $\vec x \in \Sol_\TU$, $\lambda(S,v,\vec x) = 1$ if $v(S) > \sum_{i \in S}x_i$.
%In the following table, we summarize how each of the domains discussed above maps to the elements in Definition~\ref{def:stat-solutionconcept}. We specify $\lambda$ in terms of the condition that should be satisfied. 

%\begin{tabular}{ccccc}
%\toprule
%                        & $\cal X$              & $\cal Y$      & $\Sol$    &$\lambda$ \\
%\midrule
%  Cooperative Games     & $S\subseteq N$ & $v(S)$                            & $\vec x \in \R_+^n$  & $v(S) \ge \sum_{i \in S} x_i$          \\
% \midrule
% Hedonic Games          & $S\subseteq N$ & $\left(v_i(S)\right)_{i \in S}$   & $\pi \in \Pi(N)$  & $\exists i\in S:v_i(S) \le v_i(\pi(i))$\\
% \midrule
% Competitive Equilibria & $S\subseteq G$ & $\left(v_i(S)\right)_{i \in N}$      & $\tup{\pi,\vec p}: \pi\in \Pi(G), \vec p \in \R^{|G|}$ & $\forall i \in N: v_i(\pi(i)) - \sum_{g_j \in \pi(i)} p_j \ge v_i(S) - \sum_{g_j \in S}p_j$\\
%\bottomrule
%\end{tabular}
As in the PAC learning domain, we use {\em training data} to compute solutions. 
\begin{definition}
Given an $m$-sized batch (of \textit{training data}) $T_m \in (\cal X \times \cal Y)^m$ and a $g \in \G$,
we say that $g \vdash T_m$, or ``$g$ {\em satisfies} $T_m$'', if for all $(x_i, y_i) \in T_m$, $g(x_i) = y_i$. 
The set of elements in $\G$ satisfying $T_m$ is denoted $\G_{|T_m} = \lbrace g \in \G : g \vdash T_m \rbrace$.
\end{definition}
For example, in the case of competitive equilibria, $\G_{|T_m}$ is the set of all player valuations that are consistent with the data $T_m$. 

We make the minor assumption that there is always some $g \in \G$ for which $T_m = \left(\tup{x_j,g(x_j)}\right)_{j = 1}^m$.
From now on, we identify $T_m$ with $x_1,\dots,x_m \in \cal X$.



It would often be convenient to consider problems where one can always find a consistent solution.
\begin{definition}\label{def:realizable}
A \probleminstancename problem $\probleminstance$ is called \textit{realizable}, if we are guaranteed that for all $x \in \cal X$ and any $g \in G$, there is some $s \in \Sol$ such that $\lambda(x,g,s) = 0$.
\end{definition}
Applying Definitions~\ref{def:training-data} and \ref{def:realizable} to the case of competitive equilibria, we might ask whether for some class $\cal H$ of valuations whether one can always find a solution $\tup{\pi^*,\vec p^*}$ such that for every $S \subseteq G$, $v_i(S) - p^*(S) \le v_i(\pi^*(i)) - p^*(\pi^*(i))$ for all $i \in N$. This holds, for example, when $\cal H$ is the set of all gross-substitutes valuations.


In this work we assume realizability, unless mentioned otherwise. This assumption is relatively minor for the purpose of this paper, and is mostly made for ease of exposition. 

The non-realizable case corresponds to instances for which a solution may not exist; in this case, our algorithms should output solutions that minimize {\em empirical error} as measured by $\lambda$: in other words, we seek solutions that agree with as many observed elements as possible. In the classic PAC learning domain, these are function approximations that correctly label as many datapoints as possible; in the language of our model, a candidate that beats a maximal number of observed candidates is a solution to the non-realizable version of the Condorcet problem. 

\subsection{Consistent Solvers and Barriers of Indistinguishability}\label{subsec:eq-consistency}
Good solutions are ones that minimize some notion of loss. We analyze two important notions of loss in our domain, the {\em empirical loss} and the {\em statistical loss}. 
\begin{definition}\label{def:stat-loss}
We are given an instance of the \probleminstancename problem, a latent function $g \in \G$, and a distribution $\cal D$ over $\cal X$. An $\eps$-PAC solution (w.r.t. $\cal D$ and $g$) is an element $s^*\in \Sol_{\probleminstance}$ for which
\begin{align*}
    \E_{x \sim \cal X}[\lambda(x,g,s^*)] = \Pr_{x \sim \cal X}[\lambda(x,g,s^*) = 1]< \eps
\end{align*}
\end{definition}
\begin{definition}\label{def:empirical-loss}
Given latent function $g \in \G$ and a batch of {\em training data} $T \in (\cal X \times \cal Y)^*$ such that $g \vdash T$, the empirical loss function $\Tilde{\Lambda}_{g,T}: \Sol \rightarrow [0,1]$ is given by 
\begin{align*}
\Tilde{\Lambda}_{g,T}(s) = \frac{1}{|T|} \sum\limits_{(x_j,y_j) \in T} \lambda(x_j, g, s)
\end{align*}
\end{definition}

\noindent An algorithm $\mathcal{A}_m : (\cal X \times \cal Y)^m \rightarrow \Sol$ is said to be a {\em consistent solver} for the \probleminstancename problem $\probleminstance$ if $$\forall T_m \in (\cal X \times \cal Y)^m: \forall g \in \G_{|T_m} : \forall (x_j, y_j) \in T_m: \lambda(x_j, g, \mathcal{A}_m(T_m)) = 0.$$
or equivalently,
$$\forall T_m \in (\cal X \times \cal Y)^m: \forall g \in \G_{|T_m} : \Tilde{\Lambda}_{g, T_m}(\mathcal{A}_m(T_m)) = 0$$
In other words, for any input batch $T_m$, the algorithm returns a solution that has zero loss on all instance points $x_j$'s present in batch, with respect to all functions in $\G$ that satisfy the batch.

An algorithm $\cal A$ that {\em PAC learns a solution} for a problem instance $\probleminstance$ of \probleminstancename takes as input $m\ge m_0$ i.i.d. samples $T_m \in (\cal X \times \cal Y)^m$ from some distribution $\cal D$ over $\cal X\times \cal Y$, and outputs a solution $s^* \in \Sol$. $\cal A$ satisfies the $(\eps,\delta)$ PAC solution guarantee: with probability $\ge 1- \delta$ (over the i.i.d. sampling of $T_m$), we have that 
\begin{align*}
    \Pr_{x \sim \cal D}[\lambda(x,g,s^*) = 1] < \eps
\end{align*}
for any $g \in \G$ that is consistent with $T_m$. The lower bound $m_0$ is the {\em sample complexity} of $\cal A$, and should be polynomial in $\frac1\eps$ and $\log\frac1\delta$.

We begin by showing that efficient PAC solving implies consistent solving. 
\begin{theorem}\label{thm:eq-consistency}
For a \probleminstancename $\probleminstance$, if a PAC solver exists, then a randomized consistent solver exists.
\end{theorem}

\begin{proof}
We construct a randomized consistent solver given a PAC solver $\cal A$, which outputs a consistent solution with probability $\ge \frac23$. It is easy to construct a solver that outputs such a solution with an arbitrarily higher probability using one that outputs one with a constant probability (this is a classic result on randomized algorithms). 

Given $m$ input samples $T_m$, we provide a construction for $T_{m'}$ for passing to the PAC solver subroutine. Let the consistent solver define a distribution $\cal D$ uniformly over the multiset $T_m$. The solver then invokes the PAC solver with $\eps_0 = \frac{1}{2m}$ and $\delta = \frac{1}{3}$, by sampling the points $x_j\in T_m$ from $T_m$ with this distribution (i.e. uniformly).  
If there is some $x_j \in T_m$ for which $\lambda(x_j,g,s)=1$, then $\Pr_{x \sim \cal D}[\lambda(x,g,s) = 1] \ge \frac1m>\eps_0$.
Therefore, if $\underset{X \sim \mathcal{D}}{E}[\lambda(X,g,s)] \leq \eps_0$ then $\forall x_i \in T_m: \lambda(x,g,s) = 0$.
Let $m_{\cal A}(\frac1{2m},\frac13)$ be the number of samples required by the PAC solver $\cal A$ to output a PAC solution $s^*$ with $\eps = \frac{1}{2m}$ and $\delta = \frac13$. Then, for all $g \in \G_{|T_m}$, with probability $< \frac13$, we have that  
$$\Pr_{x \sim \cal D}\E[\lambda(X, g, s^*)] > \eps_0.$$
This implies that for all $g \in \G_{|T_m}$, 
$$\Pr[\forall (x_i,y_i)\in T_m: \lambda(x_i,g,s^*) = 0]> \frac23$$

\end{proof}
To conclude, the {\em sample complexity} of a \probleminstancename problem $\probleminstance$ is the running time of the most efficient PAC solver for $\probleminstance$, and is denoted $m(\probleminstance)$. In what follows, we provide lower and upper bounds on $m(\probleminstance)$. 


\subsection{Lower Bounds on Sample Complexity}\label{subsec:lower-bound}
In this section, we present novel definitions of dimension that can be employed in the PAC solution setting.  
\begin{definition}\label{def:pac-reduct}
A \probleminstancename problem $\probleminstance$ is said to be \textit{PAC reducible} to a \probleminstancename problem $\probleminstance'$, if 
\begin{itemize}
    \item There exists a transformation $\gamma: \cal X \times \cal Y \rightarrow \cal X' \times \cal Y'$, that takes single sample from $\probleminstance$ to single samples in $\probleminstance'$, such that it transforms any legitimate batch in $\probleminstance$ (ie. there exists some latent function $g \in \G$ that satisfies it) into a legitimate batch for $\probleminstance'$.
    \item There exists a correspondence $\beta: \Sol' \rightarrow \Sol$, such that any solution in $\probleminstance'$ can be used to construct a solution in $\probleminstance'$, without any additional potential statistical loss.
\end{itemize}
\end{definition}
As one would expect, PAC reductions preserve sample complexity. The following straightforward lemma is given without proof.  
\begin{lemma}\label{lemma:pac-reduct}
If $\probleminstance'$ is PAC reducible to $\probleminstance$, and there exists a PAC solver $\cal L$ for $\probleminstance$ with sample complexity $m_{\mathcal{L}}(\eps, \delta)$, then there exists a PAC solver $\mathcal{L}'$ for $\probleminstance'$ such that (for all $\eps$ and $\delta$) $m_{\mathcal{L}'}(\eps, \delta) \leq m_{\mathcal{L}}(\eps, \delta)$.
\end{lemma}
In order to lower-bound the dimension of a \probleminstancename problem, we employ variants of the classic Natarajan dimension \cite{natarajan1989learning}.
\begin{definition}[Generalized Natarajan Dimension]\label{def:gen-n-dim}
Given a set of samples $C \subseteq \cal X$, we say that $C$ is N-shattered in a $\probleminstancename$ problem $\probleminstance$, if there exist some $g_0, g_1 \in \G$, such that $g_0(x) \ne g_1(x)$ for all $x \in C$, and for every binary labeling $b:C \to \{0,1\}$, there is a solution $s_b \in \Sol$ such that for all $x \in C$: 
$$\lambda(x,g_0,s_b) = b(x); \lambda(x,g_1,s_b) = 1- b(x).$$
%$$(\forall x \in B: \lambda(x,g_0,s_B) = 0 \wedge \lambda(x,g_1,s_B) = 1) \wedge (\forall x \in C \setminus B: \lambda(x,g_0,s) = 1 \wedge \lambda(x,g_1,s) = 0)$$.
The generalized Natarajan dimension of a $\probleminstancename$ problem $\probleminstance$ (denoted $d_N(\probleminstance$) is the size of the largest set that is N-shattered under $\probleminstance$. The set $C$ and its corresponding functions $g_0,g_1$ are referred to as the {\em shattering witness}. 
\end{definition}
We now generalize a result from \citet{daniely2011multiclass} to show that the sample complexity of a problem $\probleminstance$ is lower bounded by $d_N(\probleminstance)$.
\begin{theorem}\label{thm:lower-bound}
(generalization of lower bound result from \cite[Theorem 4]{daniely2011multiclass}) 
There is a universal constant $\alpha_1$, such that for all $\probleminstance$, if $\mathcal{L}$ is a PAC solver for it, then
$$m_{\mathcal{L}}(\eps, \delta) \geq \frac{\alpha_1}{\eps}(d_N(\probleminstance) + ln(\frac{1}{\delta}))$$
\end{theorem}

\begin{proof}
Let $\tup{C, g_0, g_1}$ be the shattering witness for $\probleminstance$. 

For each $s \in \Sol$, we define $\phi_s: C \rightarrow \lbrace 0,1 \rbrace$ as follows:
\begin{align*}
\phi_s(x) = 
\begin{cases}
0 & \text{if }\lambda(x,g_0,s)=0,\\
1 & \text{otherwise}
\end{cases}
\end{align*}

Learning $\phi_s$ is PAC reducible to $\probleminstance$, under the transformation $\gamma : (x, i) \mapsto (x, g_i(x))$. Also, observe that the set of $\phi_s$'s have VC dimension equal to the generalized Natarajan dimension of $\probleminstance$. Since sample complexity of any PAC learner for $\phi_s$'s is lower bounded, the same lower bound therefore also applies to any PAC solver of $\probleminstance$.
\begin{yaircomment}
	This needs more detail
\end{yaircomment}
\end{proof}

\iffalse
\begin{definition}
Given a function $f \in \cal Y^C$, for a subset $C \subseteq \cal X$, and a $g \in \G$,
\begin{itemize}
    \item We say that $g \vdash f$, or \textit{``$g$ satisfies $f$''}, if $\forall x \in C: f(x) = g(x)$,
    \item and, $\G_{|f} = \lbrace g \in \G: g \vdash f \rbrace$.
\end{itemize}
\end{definition}
\fi


\subsection{Upper Bound on Sample Complexity via ERM Principle}
We now turn to presenting an upper bound on the sample complexity of solution learning, via the {\em graph dimension} of $\probleminstance$.

\begin{definition}\label{def:G-shattering}
Let $C \subseteq \cal X$, we say the set $C$ is G-shattered in $\probleminstance$ if there exists a $g \in \G$, such that for every binary labeling $b:C \to \{0,1\}$ there exists a solution $s \in \Sol$ (that may depend on $b$) such that for all $x \in C$, $\lambda(x,g,s) = b(x)$.

The generalized graph dimension of $\probleminstance$, denoted $d_G(\probleminstance)$ is the size of the largest set G-shattered in $\probleminstance$, and $(C, g)$ as the corresponding shattering witness.
\end{definition}

Indeed, the graph dimension $d_G(\probleminstance)$ serves as an upper bound on the sample complexity of $\probleminstance$.

\begin{theorem} \label{thm:upperbound}
There is a universal constant $\alpha_2$, such that for any $\probleminstance$, for any batch (of sampled training data) $T_m$, generated by some $g \in \G$, and sampled with distribution $\mathcal{D}^m$, such that
$$m > \frac{\alpha_2}{\eps} \left( ln(\frac{1}{\delta}) + d_{G}(\probleminstance) ln(\frac{1}{\eps})\right)$$
if a solution $s \in \Sol$ is consistent with the batch, then it is an $(\eps, \delta)$-PAC solution as well.

Equivalently, if there exists a consistent solver $\mathcal{A}$ for $\probleminstance$, then it is also a PAC solver with sample complexity
$$m_{\mathcal{A}}(\eps, \delta) \leq \left(\frac{\alpha_2}{\eps}\right) \left( ln(\frac{1}{\delta} + d_{G}(\probleminstance) ln(\frac{1}{\eps})\right)$$
\end{theorem}


\begin{proof}
For any $g \in \G$, consider $\Phi_g = \lbrace \phi_{g,s}: \cal X \rightarrow \lbrace 0,1 \rbrace | s \in \Sol, \phi_{g,s} (x) = 1 - \lambda(x, g, s) \rbrace$. Observe that, $d_G(\probleminstance) = \underset{g}{max} \, \VC(\Phi_g)$; this implies that if $d_G(\probleminstance) = d$, then for every $g \in \G$, $|\Phi_g| \leq |\cal X|^d$.

If $\Ind: \cal X \rightarrow \lbrace 0,1 \rbrace$, such that $\forall x: \Ind(x) = 1$, then by realizability we know that $\forall g \in \G: \Ind \in \Phi_g$. Also, $\Lambda_{g, \mathcal{D}} (s) = dist_{\mathcal{D}}(\phi_{g,s}, \Ind)$. Since, an ERM solver always provides a solution $s \in \Sol$ that ensures $\phi_{g,s}$ is equal to $1$ for all sample points $x_i$(s), therefore the upper bound follows from the uniform convergence of binary classifiers in $\Phi_g$.
\end{proof}

Theorem~\ref{thm:upperbound} is a subtle yet crucial departure from the corresponding result in simple learning, where the existence of a consistent learner is guaranteed. In the realizable case of simple learning, it is always possible to find a hypothesis that consistently fits the training data by a brute force search. However, the above theorem is conditioned by the existence of a consistent solver, which may not always exist.
Indeed, the non-existence of a consistent solver precludes us from finding a PAC solution for competitive equilibria under linear utilities; a similar result yields non-existence of a PAC core solution for additive hedonic games \cite{sliwinski2017hedonic}. In both cases, a solution is guaranteed to exist, but a solver cannot identify it with arbitrarily high probability. 

To conclude, in order to establish efficient PAC algorithm for a problem $\probleminstance$, it suffices to upper-bound $m(\probleminstance)$ by its generalized graph dimension $d_G(\probleminstance)$; in order to show that $\probleminstance$ is not PAC solvable, it suffices to lower-bound $m(\probleminstance)$ by its generalized Natarajan dimension $d_N(\probleminstance)$. In what follows, we show how this technique can be used to establish the PAC learnability of various solution concepts from the EconCS literature. 
